RoBIC: A benchmark suite for assessing classifiers robustness

Many defenses have emerged with the development of adversarial attacks. Models must be objectively evaluated accordingly. This paper systematically tackles this concern by proposing a new parameter-free benchmark we coin RoBIC. RoBIC fairly evaluates the robustness of image classifiers using a new half-distortion measure. It gauges the robustness of the network against white and black box attacks, independently of its accuracy. RoBIC is faster than the other available benchmarks. We present the significant differences in the robustness of 16 recent models as assessed by RoBIC.

==> 2_Benchmark.tex <==
% !TEX root =  main.tex



\section{The benchmark}
\label{sec:benchmark}
This section justifies the recommendations made in our benchmark and defines the measure of robustness.

\textbf{Pixel domain.} Our benchmark is dedicated to image classification.
As a consequence, the distortion is defined on the pixel domain:
An image $I$ is defined in the space $\llbracket0,255\rrbracket^n$ with $n=3RC$ pixels for 3 color channels, $R$ rows and $L$ columns.
Most papers in the field measure distortion after the transformation of the image in a tensor $x\in\mathcal{X}^n$.
This is a mistake preventing a fair comparison: for most models $\mathcal{X}=[0,1]$, but for some others $\mathcal{X}=[-1,1]$ or $\mathcal{X}=[-3,3]$.

Our benchmark assumes that an adversarial image is above all an image, \ie\ a discrete object $I_a\in\llbracket0,255\rrbracket^n$.
Again, most attacks output a continuous tensor $x_a\in\mathcal{X}^n$, neglecting the quantization.
This is a mistake: in real-life, the attacker has no access to $x_a$, which is an auxiliary data internal of the model.

\textbf{Distortion.} The distortion is defined as the root mean square error: $d(I_a,I_o) := \|I_a - I_o\|_2 / \sqrt{n}$. 
This is easily interpretable: if $I_{a,i} = I_{o,i} \pm \epsilon$, $\forall i\in\llbracket 1,n\rrbracket$, then $d(I_o,I_a)=\epsilon$.
It is easily translated into a PNSR as image processing professionals do: $\mathrm{PSNR} = 48.13 - 20\log_{10}(d(I_o,I_a))$ dB.
Adversarial perturbations usually spread all over the image and have small amplitude like in invisible watermarking.
This is a case where measures based on $\ell_2$ norm remain good indicators of the quality.  
A perceptual similarity is obviously better, but more complex and less interpretable.
 
\textbf{Test set.} The input of the model is a natural and large image. Assessing the robustness of models on specific dataset like MNIST (almost black and white), or on tiny images like CIFAR does not reflect the complexity of the problem. Our benchmark considers natural images of at least $224\times 224$ pixels as provided in ImageNet.
The test set is a secret subset of $1000$ images. Otherwise, attackers or defenders may tweak their algorithms for a particular set.    

\textbf{Operating characteristic.} An attack is a process outputting an image $I_a = \Att(I_o, M, \Pi)$, where $I_o$ is the original image, $M$ is the target model, and $\Pi$ is a set of attack parameters.
The ground truth label of $I_o$ is denoted by $y_o$.
The boolean function $\mathbb{1}(I_a,y_o) = [M(I_a)\neq y_o]$ indicates whether the attack deludes model $M$ in the untargeted attack scenario: the predicted class $M(I_a)$ is different than the ground truth.

The game between attack $\Att$ and model $M$ over the test set is summarized by the operating characteristic $D\to P(D)$ relating the distortion $D$ and the probability of success $P(D)$:
\begin{equation}
P(D) := n^{-1}\sum_{i: d(I_{a,i},I_{o,i})\leq D }^{n} \mathbb{1}(I_{a,i},y_{o,i}).
\end{equation}
In other words, $P(D)$ is the fraction of images that the attack succeeded to hack within a distortion budget $D$. 
Alternatively, a defender is interested in the accuracy function $\acc(D) := 1-P(D)$. 
The value $\eta(0)$ is the classical accuracy of the model over original images. %measuring its generalization.
Function $\eta(D)$ is by construction non increasing and should converge to 0 as the distortion $D$ increases.
%This function allows a fair comparison of white-box or black-box attacks. 

\textbf{Measure of robustness.} After observing many accuracy functions for different models and attacks, we notice that they share the same prototype:
\begin{equation}
\acc(D) = \acc(0)~e^{-\lambda D} \quad \text{with }  \lambda \in \mathbb{R^+}.
\end{equation}
Like in nuclear physics, we define the half-distortion $\hd$ as the distortion needed to reduce to half the initial accuracy:
\begin{equation}
\label{eq:HD}
\acc(\hd) = \acc(0)/2,\quad \hd = \lambda^{-1}\log(2).
\end{equation}

 
This approximation is verified experimentally with an average coefficient of determination $R^2$ of 99\%.
The half-distortion $\hd$ will be the keystone of the proposed metric of robustness.
A model is then characterized by three separated concepts: its generalization ability $\acc(0)$ and its robustnesses $\hd$ against black-box and white-box attacks.

 


==> 3_Difficulties.tex <==
% !TEX root =  main.tex

\section{Difficulties}
\label{sec:difficulties}
The half distortion is a statistics extracted from the adversarial images forged from the test set.
It depends on the attack $\Att$ and its set of parameters $\Pi$.
Therefore, it can not play the role of a measure of robustness of a given model.
The first problem is to get rid off the impact of parameters $\Pi$.

\subsection{The best effort mode}
As mentioned in the introduction, parameters $\Pi$ have a huge impact on the power of an attack.
For instance, some attacks like \fgsm, \ifgsm, \pgd are distortion constrained in the sense that $\Pi$ is strongly connected to a distortion budget.
If the distortion budget is small, the probability of the success of the attack is small. If it is large, this probability is close to 1 but the distortion is too big.
Hence, it is hard to find the best setting to make these attacks competitive.

Our strategy, so-called `best effort mode', reveals the intrinsic power of an attack by finding the best setting for any image: $I_a = \Att(I_o, M, \Pi^\star)$ with
\begin{equation}
\Pi^\star = \arg\min_{\Pi:\mathbb{1}(\Att(I_o, M, \Pi),y_{o})=1} d(\Att(I_o, M, \Pi),I_o).
\end{equation}
%This is typically done with a grid search to find the necessary but sufficient distortion per image needed by this attack.
The best effort mode makes the measurement of $\hd$ independent from an arbitrary setting $\Pi$.
Yet, it is costly in terms of computations. Attacks with few parameters are preferred.

\subsection{Worst case attacks}
A second difficulty is to make $\hd$ independent of the attack.
Ideally, we would like to know the worst case attack in order to certify the robustness of a model. 
An option proposed by benchmarks \robustvision and \ares is to consider a set of $J$ attacks.
%In our framework, this would redefine the half distortion over the envelope of $J$ accuracy functions:
%\begin{equation}
%\acc(D) = \min_{1\leq j \leq J} \acc_{\Att_j}(D), \quad\forall D>0.
%\end{equation}
This is again costly as each image of the test set has to be attacked $J$ times.
Yet, a benchmark happens to be useful if it is fast enough so to assess the robustness of many models.
The best effort mode over an ensemble of attacks is out of reach.
This is the reason why we need to focus on fast worst case attacks in the sense that they achieve their best effort mode within limited complexity.  

==> 6_Notes.tex <==
% !TEX root =  main.tex
\section{Notes de preparation}
Liste des benchmarks concurrents:

\begin{itemize}
\item ADBD: \rays also proposes ADBD (Average Distance to Boundary Decision) as a measure of robustness.
It is based on $L_\infty$, 1000 CIFAR-10 images, black-box only 4000 queries. see \url{https://github.com/uclaml/RayS}.
\item RobustBench~\cite{Croce:2020aa}: standardized benchmark (no adaptive attacks), $L_\infty$ or $L_2$ attacks, mostly CIFAR10.
Measure = Adversarial accuracy under a given $\epsilon$ distortion budget. \url{https://robustbench.github.io/}. Pipeline of attacks, remove attacks if previous success to attack.
\item Robust Vision Benchmark: \url{github.com/bethgelab/robust-vision-benchmark} or \url{https://robust.vision/benchmark/leaderboard/}. 
Best Effort for a	 given attack. Measure = median of $L_2$ norm over all attacks in best effort. ImageNet.
11 attacks, results not clear.
\item ARES~\cite{Dong:2020aa} \url{https://github.com/thu-ml/ares}. Still under development but there is 11 attacks
Many curves: one curve for each model for each attacks.
Show curves: accuracy vs perturbation budget and accuracy vs attack strength
	-
\item Robust-ML:  \url{https://github.com/robust-ml/robustml}. Adaptive attacks. 
specific benchmark. Only CW is used (see robustbench paper) and the parameters are fitted manually for each model. It's not really to compare models and defenses but more Carlini wagner

\end{itemize}•

\begin{table}[h]
	\centering
	\resizebox{\linewidth}{!}{%
		\setlength\tabcolsep{2pt}
		\begin{tabular}{|c|c|c|c|c|c|c|}
			\hline
			& \multicolumn{2}{|c|}{Our} & \multicolumn{2}{|c|}{RobustBench~\cite{Croce:2020aa}} & \multicolumn{2}{|c|}{ADBD~\cite{Chen:2020ab}} \\
			Model & Time & Score & Time & Score & Time & Score \\
			\hline
			AlexNet~\cite{DBLP:journals/corr/Krizhevsky14} & 59 min & 2.17 & \textbf{2 min} & 0\% & 450 min & 0.0018 \\
			\hline
			EfficientNet~\cite{pmlr-v97-tan19a} & 61 min & 3.56 & \textbf{7 min} & 2\% & 830 min & 0.0057 \\
			\hline
			ResNet50~\cite{madry2018towards} & \textbf{73 min} & 9.88 & 80 min & 56\% & Too long & \\ 
			\hline
		\end{tabular}
	}
	\caption{Runtimes to evaluate the robustness of a model with 100 ImageNet images.}
	\label{table:benchmark_runtimes}
\end{table}

\textbf{Runtimes}: we compare our runtime with \robustbench with $\ell_2=0.5$ and ADBD run with $40000$ queries. \robustvision and \robustml are missing in this comparison because the parameters or attacks are not clearly given. We evaluate them on 100 ImageNet images.

In table \ref{table:benchmark_runtimes}, \robustbench is faster than us on AlexNet~\cite{DBLP:journals/corr/Krizhevsky14} and EfficientNet~\cite{pmlr-v97-tan19a}.
Its pipeline makes the benchmark faster by removing images that have already been successfully attacked. If the model is not very robust, like AlexNet, it could be very fast. 
However, this stategy this strategy is not as useful if the model is robust. For example, they is slower than ours for ResNet50~\cite{madry2018towards}.

They also set a distance $\ell_p$ to remove images below this distance. \ares and \robustml have this too. But its arbitrarily fixed to $\ell_2=0.5$ and $\ell_{\infty}=8/255$. The smaller this fixed distance is, the more challenging but slower the benchmark will be.
We decided to establish an objective measure by the half-life. This allows us to have a finer vision of the robustness, but require to attack all the images.

Moreover, except the different runtime, all the different benchmark in \ref{table:benchmark_runtimes} give the same ranking.\\


==> 7_Notes.tex <==
% !TEX root =  main.tex
\section{Notes de preparation}
Liste des benchmarks concurrents:

\begin{itemize}
\item ADBD: \rays also proposes ADBD (Average Distance to Boundary Decision) as a measure of robustness.
It is based on $L_\infty$, 1000 CIFAR-10 images, black-box only 4000 queries. see \url{https://github.com/uclaml/RayS}.
\item RobustBench~\cite{Croce:2020aa}: standardized benchmark (no adaptive attacks), $L_\infty$ or $L_2$ attacks, mostly CIFAR10.
Measure = Adversarial accuracy under a given $\epsilon$ distortion budget. \url{https://robustbench.github.io/}. Pipeline of attacks, remove attacks if previous success to attack.
\item Robust Vision Benchmark: \url{github.com/bethgelab/robust-vision-benchmark} or \url{https://robust.vision/benchmark/leaderboard/}. 
Best Effort for a	 given attack. Measure = median of $L_2$ norm over all attacks in best effort. ImageNet.
11 attacks, results not clear.
\item ARES~\cite{Dong:2020aa} \url{https://github.com/thu-ml/ares}. Still under development but there is 11 attacks
Many curves: one curve for each model for each attacks.
Show curves: accuracy vs perturbation budget and accuracy vs attack strength
	-
\item Robust-ML:  \url{https://github.com/robust-ml/robustml}. Adaptive attacks. 
specific benchmark. Only CW is used (see robustbench paper) and the parameters are fitted manually for each model. It's not really to compare models and defenses but more Carlini wagner

\end{itemize}•

\begin{table}[h]
	\centering
	\resizebox{\linewidth}{!}{%
		\setlength\tabcolsep{2pt}
		\begin{tabular}{|c|c|c|c|c|c|c|}
			\hline
			& \multicolumn{2}{|c|}{Our} & \multicolumn{2}{|c|}{RobustBench~\cite{Croce:2020aa}} & \multicolumn{2}{|c|}{ADBD~\cite{Chen:2020ab}} \\
			Model & Time & Score & Time & Score & Time & Score \\
			\hline
			AlexNet~\cite{DBLP:journals/corr/Krizhevsky14} & 59 min & 2.17 & \textbf{2 min} & 0\% & 450 min & 0.0018 \\
			\hline
			EfficientNet~\cite{pmlr-v97-tan19a} & 61 min & 3.56 & \textbf{7 min} & 2\% & 830 min & 0.0057 \\
			\hline
			ResNet50~\cite{madry2018towards} & \textbf{73 min} & 9.88 & 80 min & 56\% & Too long & \\ 
			\hline
		\end{tabular}
	}
	\caption{Runtimes to evaluate the robustness of a model with 100 ImageNet images.}
	\label{table:benchmark_runtimes}
\end{table}

\textbf{Runtimes}: we compare our runtime with \robustbench with $\ell_2=0.5$ and ADBD run with $40000$ queries. \robustvision and \robustml are missing in this comparison because the parameters or attacks are not clearly given. We evaluate them on 100 ImageNet images.

In table \ref{table:benchmark_runtimes}, \robustbench is faster than us on AlexNet~\cite{DBLP:journals/corr/Krizhevsky14} and EfficientNet~\cite{pmlr-v97-tan19a}.
Its pipeline makes the benchmark faster by removing images that have already been successfully attacked. If the model is not very robust, like AlexNet, it could be very fast. 
However, this stategy this strategy is not as useful if the model is robust. For example, they is slower than ours for ResNet50~\cite{madry2018towards}.

They also set a distance $\ell_p$ to remove images below this distance. \ares and \robustml have this too. But its arbitrarily fixed to $\ell_2=0.5$ and $\ell_{\infty}=8/255$. The smaller this fixed distance is, the more challenging but slower the benchmark will be.
We decided to establish an objective measure by the half-life. This allows us to have a finer vision of the robustness, but require to attack all the images.

Moreover, except the different runtime, all the different benchmark in \ref{table:benchmark_runtimes} give the same ranking.\\

